Faster Fundamental Graph Algorithms via Learned Predictions

We consider the question of speeding up classic graph algorithms with machine-learned predictions. In this model, algorithms are furnished with extra advice learned from past or similar instances. Given the additional information, we aim to improve upon the traditional worst-case run-time guarantees. Our contributions are the following: (i) We give a faster algorithm for minimum-weight bipartite matching via learned duals, improving the recent result by Dinitz, Im, Lavastida, Moseley and Vassilvitskii (NeurIPS, 2021); (ii) We extend the learned dual approach to the single-source shortest path problem (with negative edge lengths), achieving an almost linear runtime given sufficiently accurate predictions which improves upon the classic fastest algorithm due to Goldberg (SIAM J. Comput., 1995); (iii) We provide a general reduction-based framework for learning-based graph algorithms, leading to new algorithms for degree-constrained subgraph and minimum-cost $0$-$1$ flow, based on reductions to bipartite matching and the shortest path problem. Finally, we give a set of general learnability theorems, showing that the predictions required by our algorithms can be efficiently learned in a PAC fashion.

==> push_relabel.tex <==
\subsection{Push-relabel algorithms}
The push-relabel algorithm maintains a ``preflow'' and a set of vertex heights and is built off of two main primitives: push and relabel operations.

\begin{definition}[preflow]
Given a graph $G=(V,E)$ with non-negative edge capacities $\{c_e: e \in E\}$, a \emph{preflow} $\{f_e: e \in E\}$ is an assignment of weights to the edges with the following conditions:
\begin{itemize}
    \item (non-negativity) $f_e \geq 0$ for all $e \in E$
    \item (capacity) $f_e \leq c_e$ for all $e \in E$
    \item (weak conservation) $\sum_{e \in \delta^+(v)} f_e \leq \sum_{e \in \delta^-(v)} f_e$ for all $v \in V$ ($\delta^-(v)$ indicates the edges coming into $v$ and $\delta^+(v)$ indivates the edges leaving $v$)
\end{itemize}
\end{definition}

\begin{definition}[labeling]
Given a graph $G=(V,E)$, a preflow $f$, and source/sink vertices $s,t$, let $G_f=(V,E_f)$ be the residual graph of $G$ induced by $f$. Then, $\{h_v: v \in V\}$ is a \emph{valid labeling} of the nodes in $G_f$ if
\begin{itemize}
    \item (source/sink) $h_s = n$ and $h_t = 0$
    \item (non-negativity) $h_v \geq 0$ for all $v \in V$
    \item (downhill by at most one) $h_u \leq h_v + 1$ for all $(u,v) \in E_f$ where $u,v \neq V \setminus \{s,t\}$
\end{itemize}
\end{definition}

A result of this definition is the following fact:
\begin{fact}
$h_v$ is a lower bound on the shortest path distance from $v$ to $t$ in the residual graph $G_f$.
\end{fact}
This is because along each edge in the residual graph, heights decrease by at most one. The result follows from the fact that $h_t = 0$ and heights are non-negative.
We can strengthen the connection between shortest paths and labelings with the following lemma (used in the so called ``global relabeling'' heuristic for push-relabel algorithms).
\begin{lemma}[shortest path labeling]
The assignment $h_v = d_{G_f}(v,t)$ for all $v \in V \setminus \{s,t\}$ where $d_{G}(u,v)$ is the shortest path distance from $u$ to $v$ in $G$ (or $n$ if $u,v$ are disconnected) is a valid labeling.
\end{lemma}
\begin{proof}
Consider any node $u \in V \setminus \{s,t\}$. $h_v$ is always non-negative, so we just need to check that for all of its outgoing edges go downhill by at most 1.
Consider any edge $u, v \in E_f$.
As, $d_{G_f}(u,t) \leq 1 + d_{G_f}(v,t)$, the constraint is satisfied.
\end{proof}

\subsection{Algorithm}

\paragraph{Initialization} We start off with a preflow that saturates all edges outgoing from the source $s$ and sends zero flow along any other edges.
The initial labeling sets $h_s = n$ and $h_u = 0$ for all $u \neq s$.

\paragraph{Active vertices} A vertex $u$ is called ``active'' if it has positive excess (flow in minus flow out) and has height $h_u < n$.
If there are no active vertices, we are done with the first stage of the algorithm and will move on to stage 2.
If there are active vertices, pick the active vertex $u$ with the largest height (this choice called Highest Label or HL yields a more efficient algorithm than picking an arbitrary vertex).
If possible, $Push(u)$. Else, $Relabel(u)$.

\paragraph{Push}
An edge $(u,v) \in E_f$ is ``admissible'' if $h_u = h_v +1$.
If $u$ has an admissible outgoing edge $(u,v)$, we are allowed to push flow from $u$ to $v$.
We will push the maximum amount of flow we can, bounded by the minimum of the excess flow at $u$ and the capacity of $(u,v)$.

\paragraph{Relabel}
If we could not push on $u$, we will relabel.
Set
\[
    h_u = \min\left(n, 1 + \min_{v: (u,v) \in E_f} h_v\right)
\]
(i.e. the smallest height such that $u$ has an admissible edge or $n$ otherwise).

\paragraph{Stage Two}
Once stage one is complete (push-relabel steps) and there are no more active vertices, then the vertices $\{u: h_u = n\}$ form the $s$-side and the vertices $\{u: h_u < n\}$ form the $t$-side of the $s-t$ min cut.
In addition, all nodes on the $t$-side will have no excess.
Therefore, the only remaining job is to remove the excess on the $s$-side by sending flow back to $s$ from nodes with excess.

First, we will make the preflow acyclic. This can be done in $O(m\log n)$ time via dynamic trees~\cite{sleator1983data}.
Consider the graph $H$ whose vertices are the $s$-side of the cut and whose edges represent the acyclic preflow $f$.
$H$ is a DAG and by sending excess flow in reverse topological order, we can remove all excess without changing the flow value (as conservation is maintained and all of the cut edges are still saturated).
It will take linear time to build the topological order and then to remove excess.
So, the runtime of Push-Relabel will be dominated by the first stage where we find the cut via push/relabel operations.

\Justin{There are also single stage versions of the algorithm where we don't cap the heights to $n$ and just keep running push-relabel ops until there are no active vertices. From prior work, the two stage version seems to be better in practice.}

\subsection{Correctness}

See proof in references. As long as a valid preflow and labeling is maintained and the algorithm terminates, we will end up with a max flow.

\subsection{Runtime analysis}

The runtime analysis will be split into three parts: analyzing the number of relabel operations, the number of ``saturating'' push operations, and the number of ``non-saturating'' push operations.

\begin{definition}
A push operation is called ``saturating'' if it saturates the capacity constraint of the edge it pushes along. Otherwise, the push operation is called ``non-saturating'' and must have been constrained by the amount of excess at the node it was pushing from.
\end{definition}

\begin{lemma}
The number of relabel operations is at most $n^2$.
\end{lemma}
\begin{proof}
Whenever a node is relabeled, it's height increases by at least one. As there are $n$ nodes with max height $n$, there can be at most $n^2$ relabel operations.
\end{proof}

\begin{lemma}
The number of saturating pushes is at most $mn/2$.
\end{lemma}
\begin{proof}
Consider any edge $(u,v)$.
If a push from $u$ saturates $(u,v)$, then $d_u = d_v + 1$ and $(u,v)$ disappears from the residual graph.
In order for the edge to reappear, we must push flow along $(v,u)$.
In order for this to happen, $v$ must be relabeled.
Then, in order for us to be able to do another saturating push on $(u,v)$, $u$ must also be relabeled.

The number of saturating pushes on any edge $(u,v)$ is bounded by $n/2$ as each of $u, v$ must be relabeled to be higher than the other before another saturating push can occur.
The total bound on the number of saturating pushes is thus $mn/2$.
\end{proof}

\begin{lemma}
The number of non-saturating pushes is at most $n^3$.
\end{lemma}
\Justin{This can be improved to $O(n^2 \sqrt{m})$ with slightly more complex analysis, see references.}
\begin{proof}
Let a phase be defined as all pushes between two consecutive relabel operations.
Per phase, each vertex can only have one non-saturating push.
After a vertex finishes a non-saturating push, the vertex is no longer active and will only become active again once some other vertex pushes excess onto it.
However, as we push the highest active vertices first and vertices can only push excess downhill, no vertices that become unactive during this phase will become active again until some relabelings occur.
As there are $\leq n^2$ relabels, there are $\leq n^2$ phases, yielding the total bound of at most $n^3$ non-saturating pushes.
\end{proof}

\begin{theorem}
The HL push-relabel algorithm runs in time $O(n^3)$.
\end{theorem}

\subsection{Learning Preflows}

The model is that we are running max-flow on similar graphs day after day.
For now, assume that the vertices of the graph do not change, but the edge capacities do (including whether an edge has non-zero capacity).

To warm-start our algorithm, we will be given a predicted preflow $f''$ that satisfies non-negativity and weak conservation but does not necessarily satisfy capacity constraints on the new graph $G$.

\subsection{Fixing the prediction}
First, we will describe an algorithm to turn the predicted preflow $f''$ into a valid preflow on $G$.
We will assume that $f''$ is acyclic (we can turn it acylic in near-linear time either at the start of this process or beforehand using the procedure described for Stage Two above).
Now the preflow is a DAG and we will fix some topological order on the vertices.
Following this topological order from left to right, do the following when we reach vertex $u$:
\begin{itemize}
    \item For each outgoing edge $(u,v)$ where the preflow violates its capacity constraint, reduce the flow in $f''$ along $(u,v)$ s.t. $f''_{u,v} = c_{u,v}$.
    \item If $u$ does not satisfy the weak conservation constraint (because incoming edges were violated and their flow was reduced), then reduce flow on arbitrary outgoing edges from $u$ until the conservation is met with equality.
\end{itemize}
As new constraints are only violated further down the topological order, once we finish one pass over all vertices, we are done with this process taking $O(m)$ time.

At the end, we may need to resaturate all edges leaving $s$.

\Justin{This fixing process isn't optimizing anything to do with the utility of the predicted preflow, so maybe some improvements could be made by tying it to the bounds on the runtime we get below. I think we can claim the following but don't think it is very useful.}
\begin{claim}
The amount of flow into $t$ reduced from fixing $f''$ is at most the total amount $f''$ violated capacities in $G$.
\end{claim}

\subsection{Setting the labeling}
Let $f'$ now denote the fixed predicted preflow: $f'$ is a valid preflow in $G$. Then, we can simply set the labeling of the vertices in $G$ to be the shortest path distances to $t$ in $G_{f'}$. From the fact and lemma at the top of the document, this is the optimal (maximal) labeling we can give. Denote these initial labels as $\{h'_v: v \in V\}$

\subsection{Bounding the runtime in terms of the prediction}
We can now bound the runtime in terms of the heights that go along with the predicted preflow.
Let $h^*$ be an upper bound on the heights of an optimal solution (e.g., the shortest path heights of the unique max flow).
We can always set $h^*_v = n$ for all $v \neq t$ as a pessimistic upper bound.
\begin{claim}
The number of relabel operations is at most $\sum_{v \in V} h^*_v - h'_v$.
\end{claim}
As each node can only be relabeled $h^*_v - h'_v$ times to get to height $h^*_v$.

\begin{claim}
The number of saturating push operations is at most $\sum_{(u,v) \in E} \min\{h^*_u - h'_u, h^*_v - h'_v\}$.
\end{claim}
As between each saturating push on an edge, both $u$ and $v$ need to increase their heights and thus are bounded by maximum number of times we can relabel either $u$ or $v$.
(There is a factor of two to account for the fact that pushes can go in the reverse direction of edges in $E$ that cancels with a factor of $1/2$ as $u, v$ have to increase by $2$ between each saturating push.)

\begin{claim}
The number of nonsaturating push operations is at most $n \left(\sum_{v \in V} h^*_v - h'_v\right)$.
\end{claim}
As the number of phases is bounded by the number of relabels and there are at most $n$ nonsaturating pushes per phase.

\begin{theorem}
The HL push-relabel algorithm with initial heights $h'$ runs in time
\[
O\left(n \left(\sum_{v \in V} h^*_v - h'_v\right) + m\log n + n\right)
\]
\end{theorem}

\begin{proof}
The first term comes from the proceeding lemmas, and the $m\log n + n$ term comes from the second stage of push-relabel.
Note that the number of nonsaturating pushes dominates the other operations.
The number of nonsaturating pushes is a multiplicative factor of $n$ more than the number of relabels.
In addition, we can bound the number of saturating pushes as
\begin{align*}
    \sum_{(u,v) \in E} \min\{h^*_u - h'_u, h^*_v - h'_v\}
    &\leq \frac{1}{2} \sum_{v \in V} deg(v) (h^*_v - h'_v) \\
    &\leq \frac{n}{2} \sum_{v \in V} h^*_v - h'_v
\end{align*}
which is (up to constant factors) the same as the number of nonsaturating pushes.
\end{proof}

\begin{observation}
If $\sum_{v \in V} h^*_v - h'_v = o(\sqrt{n})$, this algorithm is faster than state of the art max flow algorithms.
\end{observation}

\subsection{References}
\begin{itemize}
    \item \url{https://www.cs.cmu.edu/~avrim/451f13/lectures/lect1010.pdf}
    \item \url{https://theory.stanford.edu/~tim/w16/l/l3.pdf}
    \item \url{https://cs.stanford.edu/people/trevisan/cs261/lecture12.pdf}
    \item paper with $O(n^2\sqrt{m})$ bound on HL push relabel \url{https://epubs.siam.org/doi/pdf/10.1137/0218072}
    \item Goldberg paper on heuristics for HL push relabel and description of 2-phase algorithm \url{https://link.springer.com/content/pdf/10.1007/PL00009180.pdf}
    \item Orlin empirical study of max flow algos (HL push relabel is best) \url{https://dspace.mit.edu/bitstream/handle/1721.1/2573/SWP-3811-32867587.pdf?sequence=1}
\end{itemize}

